Predictions for the hydrogen-free ejecta of pulsational pair-instability supernovae

Present time-domain astronomy efforts will unveil a variety of rare transients. We focus here on pulsational pair-instability evolution, which can result in signatures observable with electromagnetic and gravitational waves. We simulate grids of bare helium stars to characterize the resulting black hole (BH) masses and ejecta composition, velocity, and thermal state. The stars do not react "elastically" to the thermonuclear explosion: there is not a one-to-one correspondence between pair-instability driven ignition and mass ejections, causing ambiguity in what is an observable pulse. In agreement with previous studies, we find that for carbon-oxygen core masses 28Msun< M_CO<30.5Msun the explosions are not strong enough to affect the surface. With increasing mass, they first cause large radial expansion (30.5Msun<M_CO<31.4Msun), and finally, also mass ejection episodes (M_CO>31.4Msun). The lowest mass to be fully disrupted in a pair-instability supernova is M_CO=57Msun. Models with M_CO>121Msun reach the photodisintegration regime, resulting in BHs with M_BH>125Msun. If the pulsating models produce BHs via (weak) explosions, the previously-ejected material might be hit by the blast wave. We characterize the H-free circumstellar material from the pulsational pair-instability of helium cores assuming simply that the ejecta maintain a constant velocity after ejection. Our models produce He-rich ejecta with mass 10^{-3}Msun<M_CSM<40Msun. These ejecta are typically launched at a few thousand \kms and reach distances of ~10^{12}-10^{15} cm before core-collapse. The delays between mass ejection events and the final collapse span a wide and mass-dependent range (from sub-hour to 10^4 years), and the shells ejected can also collide with each other. The range of properties we find suggests a possible connection with (some) type Ibn supernovae.

==> pulses_table.tex <==
41.25 & 1 & 34.60 & \num{2.07e-05} & \num{3.22e+05} & \num{6.33e-03} & \num{3.83e+00}\\ 
\hline
42.00 & 1 & 35.14 & \num{3.29e-06} & \num{3.21e+05} & \num{1.41e-01} & \num{2.84e+00}\\ 
\hline
42.25 & 1 & 35.33 & \num{1.10e-03} & \num{3.20e+05} & \num{5.35e-01} & \num{2.45e+00}\\ 
\hline
42.50 & 1 & 35.51 & \num{9.60e-03} & \num{3.20e+05} & \num{1.26e+00} & \num{1.97e+00}\\ 
\hline
42.75 & 1 & 35.69 & \num{1.55e-02} & \num{3.19e+05} & \num{1.57e+00} & \num{1.87e+00}\\ 
\hline
43.00 & 1 & 35.87 & \num{1.48e-02} & \num{3.19e+05} & \num{1.58e+00} & \num{1.85e+00}\\ 
\hline
43.25 & 1 & 36.05 & \num{2.24e-02} & \num{3.18e+05} & \num{2.26e+00} & \num{1.77e+00}\\ 
\hline
43.50 & 1 & 36.23 & \num{1.52e+00} & \num{3.18e+05} & \num{1.05e+02} & \num{3.87e+00}\\ 
\hline
43.75 & 1 & 36.42 & \num{5.50e-01} & \num{3.17e+05} & \num{3.30e+01} & \num{3.52e+00}\\ 
\hline
44.00 & 1 & 36.59 & \num{8.73e-01} & \num{3.17e+05} & \num{7.28e+01} & \num{3.63e+00}\\ 
\hline
44.25 & 1 & 36.77 & \num{5.38e-01} & \num{3.17e+05} & \num{5.33e+01} & \num{3.27e+00}\\ 
\hline
44.50 & 1 & 36.95 & \num{5.35e-02} & \num{3.16e+05} & \num{3.78e+00} & \num{1.72e+00}\\ 
\hline
44.75 & 1 & 37.13 & \num{6.12e-02} & \num{3.16e+05} & \num{6.17e+00} & \num{1.64e+00}\\ 
\hline
45.00 & 1 & 37.31 & \num{7.43e-02} & \num{3.15e+05} & \num{7.23e+00} & \num{1.64e+00}\\ 
\hline
45.25 & 1 & 37.50 & \num{7.13e-02} & \num{3.14e+05} & \num{8.30e+00} & \num{1.61e+00}\\ 
\hline
45.50 & 1 & 37.67 & \num{8.64e-02} & \num{3.14e+05} & \num{8.51e+00} & \num{1.57e+00}\\ 
\hline
45.75 & 1 & 37.85 & \num{4.84e-02} & \num{3.14e+05} & \num{1.11e+01} & \num{1.46e+00}\\ 
\hline
46.00 & 1 & 38.03 & \num{6.38e-02} & \num{3.14e+05} & \num{1.24e+01} & \num{1.55e+00}\\ 
\hline
46.25 & 1 & 38.21 & \num{3.28e-02} & \num{3.13e+05} & \num{1.12e+01} & \num{1.37e+00}\\ 
\hline
46.50 & 1 & 38.39 & \num{2.65e-02} & \num{3.13e+05} & \num{9.71e+00} & \num{1.40e+00}\\ 
\hline
46.75 & 1 & 38.56 & \num{1.31e-01} & \num{3.12e+05} & \num{1.58e+01} & \num{1.59e+00}\\ 
\hline
47.00 & 1 & 38.74 & \num{9.25e-02} & \num{3.12e+05} & \num{1.65e+01} & \num{1.54e+00}\\ 
\hline
47.25 & 1 & 38.92 & \num{2.86e-01} & \num{3.12e+05} & \num{2.11e+01} & \num{1.66e+00}\\ 
\hline
47.50 & 1 & 39.10 & \num{4.40e-01} & \num{3.11e+05} & \num{3.00e+01} & \num{1.64e+00}\\ 
\hline
47.75 & 1 & 39.28 & \num{2.61e-02} & \num{3.11e+05} & \num{1.52e+01} & \num{1.36e+00}\\ 
\hline
48.00 & 1 & 39.45 & \num{6.11e-01} & \num{3.11e+05} & \num{5.07e+01} & \num{1.78e+00}\\ 
\hline
48.25 & 1 & 39.64 & \num{4.79e-01} & \num{3.10e+05} & \num{3.77e+01} & \num{1.56e+00}\\ 
\hline
48.75 & 1 & 39.98 & \num{8.89e-01} & \num{3.09e+05} & \num{7.55e+01} & \num{1.61e+00}\\ 
\hline
49.00 & 1 & 40.17 & \num{1.08e+00} & \num{3.09e+05} & \num{1.52e+02} & \num{1.63e+00}\\ 
\hline
49.25 & 1 & 40.34 & \num{1.14e+00} & \num{3.09e+05} & \num{1.60e+02} & \num{1.62e+00}\\ 
\hline
49.50 & 1 & 40.52 & \num{5.24e-01} & \num{3.08e+05} & \num{4.34e+01} & \num{1.78e+00}\\ 
\hline
49.75 & 1 & 40.70 & \num{1.64e+00} & \num{3.07e+05} & \num{1.80e+02} & \num{1.66e+00}\\ 
\hline
50.00 & 1 & 40.88 & \num{1.24e+00} & \num{3.07e+05} & \num{1.27e+02} & \num{1.67e+00}\\ 
\hline
50.25 & 1 & 41.05 & \num{1.84e+00} & \num{3.07e+05} & \num{2.08e+02} & \num{1.70e+00}\\ 
\hline
50.50 & 1 & 41.23 & \num{1.69e+00} & \num{3.06e+05} & \num{1.45e+02} & \num{1.78e+00}\\ 
\hline
50.75 & 1 & 41.41 & \num{1.97e+00} & \num{3.06e+05} & \num{2.13e+02} & \num{1.75e+00}\\ 
\hline
\multirow{2}{*}{51.00} & 1 & 41.58 & \num{3.98e-01} & \num{3.06e+05} & \num{3.02e+01} & \num{2.21e+00}\\ 
 & 2 & 41.18 & \num{1.61e+00} & \num{3.06e+05} & \num{1.58e+01} & \num{1.45e+00}\\ 
\hline
\multirow{2}{*}{51.25} & 1 & 41.75 & \num{4.19e-01} & \num{3.05e+05} & \num{3.19e+01} & \num{2.24e+00}\\ 
 & 2 & 41.33 & \num{1.37e+00} & \num{3.05e+05} & \num{1.74e+01} & \num{1.51e+00}\\ 
\hline
51.50 & 1 & 41.93 & \num{1.85e+00} & \num{3.05e+05} & \num{2.31e+02} & \num{1.88e+00}\\ 
\hline
\multirow{2}{*}{51.75} & 1 & 42.11 & \num{4.34e-01} & \num{3.04e+05} & \num{3.53e+01} & \num{2.11e+00}\\ 
 & 2 & 41.68 & \num{1.70e+00} & \num{3.04e+05} & \num{3.58e+01} & \num{1.64e+00}\\ 
\hline
\multirow{2}{*}{52.00} & 1 & 42.28 & \num{7.44e-01} & \num{3.04e+05} & \num{6.51e+01} & \num{2.22e+00}\\ 
 & 2 & 41.53 & \num{1.49e+00} & \num{3.04e+05} & \num{1.47e+01} & \num{1.51e+00}\\ 
\hline
52.25 & 1 & 42.46 & \num{1.47e-01} & \num{3.04e+05} & \num{1.10e+02} & \num{1.92e+00}\\ 
\hline
52.50 & 1 & 42.64 & \num{9.17e-02} & \num{3.03e+05} & \num{1.31e+02} & \num{1.60e+00}\\ 
\hline
52.75 & 1 & 42.81 & \num{3.86e-01} & \num{3.03e+05} & \num{1.69e+02} & \num{1.86e+00}\\ 
\hline
53.00 & 1 & 42.98 & \num{2.42e-01} & \num{3.03e+05} & \num{1.20e+02} & \num{1.51e+00}\\ 
\hline
53.25 & 1 & 43.16 & \num{1.18e-01} & \num{3.02e+05} & \num{6.50e+01} & \num{1.59e+00}\\ 
\hline
53.50 & 1 & 43.33 & \num{1.41e+00} & \num{3.02e+05} & \num{2.80e+02} & \num{1.99e+00}\\ 
\hline
53.75 & 1 & 43.50 & \num{1.23e+00} & \num{3.02e+05} & \num{2.40e+02} & \num{1.95e+00}\\ 
\hline
54.00 & 1 & 43.68 & \num{1.56e+00} & \num{3.01e+05} & \num{4.17e+02} & \num{1.81e+00}\\ 
\hline
54.50 & 1 & 44.03 & \num{1.75e+00} & \num{3.01e+05} & \num{3.28e+02} & \num{1.95e+00}\\ 
\hline
\multirow{2}{*}{54.75} & 1 & 44.20 & \num{1.29e+00} & \num{3.00e+05} & \num{2.03e+02} & \num{2.12e+00}\\ 
 & 2 & 42.90 & \num{5.56e-01} & \num{3.00e+05} & \num{2.38e+01} & \num{1.51e+00}\\ 
\hline
55.00 & 1 & 44.37 & \num{1.19e+00} & \num{3.00e+05} & \num{3.72e+02} & \num{1.97e+00}\\ 
\hline
\multirow{3}{*}{55.25} & 1 & 44.55 & \num{3.17e-01} & \num{3.00e+05} & \num{2.86e+00} & \num{2.19e+00}\\ 
 & 2 & 44.23 & \num{7.80e-01} & \num{3.00e+05} & \num{2.82e+02} & \num{1.85e+00}\\ 
 & 3 & 43.45 & \num{2.53e-01} & \num{3.00e+05} & \num{4.85e+01} & \num{1.49e+00}\\ 
\hline
55.50 & 1 & 44.72 & \num{1.32e+00} & \num{2.99e+05} & \num{3.51e+02} & \num{1.88e+00}\\ 
\hline
\multirow{2}{*}{55.75} & 1 & 44.89 & \num{4.42e-01} & \num{2.99e+05} & \num{4.50e+00} & \num{2.14e+00}\\ 
 & 2 & 44.45 & \num{1.06e+00} & \num{2.99e+05} & \num{1.52e+02} & \num{1.68e+00}\\ 
\hline
\multirow{2}{*}{56.00} & 1 & 45.07 & \num{5.01e-01} & \num{2.99e+05} & \num{2.76e+00} & \num{2.16e+00}\\ 
 & 2 & 44.57 & \num{1.10e+00} & \num{2.99e+05} & \num{2.31e+02} & \num{1.76e+00}\\ 
\hline
\multirow{2}{*}{56.25} & 1 & 45.24 & \num{5.18e-01} & \num{2.98e+05} & \num{2.53e+00} & \num{2.18e+00}\\ 
 & 2 & 44.72 & \num{1.13e+00} & \num{2.98e+05} & \num{1.61e+02} & \num{1.59e+00}\\ 
\hline
\multirow{2}{*}{56.50} & 1 & 45.42 & \num{6.42e-01} & \num{2.98e+05} & \num{6.19e+00} & \num{2.14e+00}\\ 
 & 2 & 44.77 & \num{7.50e-01} & \num{2.98e+05} & \num{9.11e+01} & \num{1.48e+00}\\ 
\hline
\multirow{2}{*}{56.75} & 1 & 45.59 & \num{6.26e-01} & \num{2.98e+05} & \num{5.75e+00} & \num{2.14e+00}\\ 
 & 2 & 44.96 & \num{1.81e+00} & \num{2.98e+05} & \num{1.35e+02} & \num{1.79e+00}\\ 
\hline
\multirow{2}{*}{57.00} & 1 & 45.76 & \num{6.87e-01} & \num{2.97e+05} & \num{4.64e+00} & \num{2.16e+00}\\ 
 & 2 & 45.07 & \num{1.39e+00} & \num{2.97e+05} & \num{1.25e+03} & \num{1.66e+00}\\ 
\hline
\multirow{2}{*}{57.25} & 1 & 45.93 & \num{7.37e-01} & \num{2.97e+05} & \num{8.56e+00} & \num{2.14e+00}\\ 
 & 2 & 45.19 & \num{1.58e+00} & \num{2.97e+05} & \num{1.45e+03} & \num{1.67e+00}\\ 
\hline
\multirow{2}{*}{57.50} & 1 & 46.10 & \num{8.95e-01} & \num{2.97e+05} & \num{1.74e+01} & \num{2.14e+00}\\ 
 & 2 & 45.21 & \num{1.31e+00} & \num{2.97e+05} & \num{1.03e+02} & \num{1.54e+00}\\ 
\hline
\multirow{2}{*}{57.75} & 1 & 46.27 & \num{9.93e-01} & \num{2.96e+05} & \num{2.97e+01} & \num{2.15e+00}\\ 
 & 2 & 45.28 & \num{2.22e+00} & \num{2.96e+05} & \num{2.18e+02} & \num{1.96e+00}\\ 
\hline
\multirow{2}{*}{58.00} & 1 & 46.45 & \num{1.09e+00} & \num{2.96e+05} & \num{2.91e+01} & \num{2.16e+00}\\ 
 & 2 & 45.35 & \num{2.29e+00} & \num{2.96e+05} & \num{2.34e+02} & \num{1.65e+00}\\ 
\hline
\multirow{2}{*}{58.25} & 1 & 46.62 & \num{1.16e+00} & \num{2.96e+05} & \num{3.36e+01} & \num{2.16e+00}\\ 
 & 2 & 45.45 & \num{2.90e+00} & \num{2.96e+05} & \num{6.24e+03} & \num{1.77e+00}\\ 
\hline
\multirow{2}{*}{58.50} & 1 & 46.79 & \num{1.08e+00} & \num{2.96e+05} & \num{3.36e+01} & \num{2.15e+00}\\ 
 & 2 & 45.71 & \num{1.70e+00} & \num{2.96e+05} & \num{1.50e+02} & \num{1.63e+00}\\ 
\hline
\multirow{2}{*}{58.75} & 1 & 46.96 & \num{1.29e+00} & \num{2.95e+05} & \num{3.84e+01} & \num{2.18e+00}\\ 
 & 2 & 45.67 & \num{1.68e+00} & \num{2.95e+05} & \num{4.96e+02} & \num{1.76e+00}\\ 
\hline
\multirow{2}{*}{59.00} & 1 & 47.13 & \num{1.18e+00} & \num{2.95e+05} & \num{3.38e+01} & \num{2.16e+00}\\ 
 & 2 & 45.95 & \num{3.26e+00} & \num{2.95e+05} & \num{6.32e+03} & \num{1.85e+00}\\ 
\hline
\multirow{2}{*}{59.25} & 1 & 47.31 & \num{1.45e+00} & \num{2.95e+05} & \num{3.84e+01} & \num{2.20e+00}\\ 
 & 2 & 45.86 & \num{1.69e+00} & \num{2.95e+05} & \num{4.51e+02} & \num{1.87e+00}\\ 
\hline
\multirow{3}{*}{59.50} & 1 & 47.48 & \num{1.31e+00} & \num{2.94e+05} & \num{3.63e+01} & \num{2.18e+00}\\ 
 & 2 & 46.17 & \num{1.04e+00} & \num{2.94e+05} & \num{1.47e+02} & \num{1.71e+00}\\ 
 & 3 & 44.19 & \num{4.73e-01} & \num{2.94e+05} & \num{6.90e+00} & \num{1.70e+00}\\ 
\hline
\multirow{2}{*}{59.75} & 1 & 47.65 & \num{1.50e+00} & \num{2.94e+05} & \num{3.80e+01} & \num{2.20e+00}\\ 
 & 2 & 46.15 & \num{1.61e+00} & \num{2.94e+05} & \num{2.42e+02} & \num{1.63e+00}\\ 
\hline
\multirow{3}{*}{60.25} & 1 & 48.00 & \num{1.38e+00} & \num{2.93e+05} & \num{3.76e+01} & \num{2.18e+00}\\ 
 & 2 & 46.61 & \num{1.80e+00} & \num{2.93e+05} & \num{2.28e+02} & \num{1.66e+00}\\ 
 & 3 & 44.24 & \num{1.81e-02} & \num{2.93e+05} & \num{6.15e-01} & \num{1.73e+00}\\ 
\hline
\multirow{2}{*}{60.75} & 1 & 48.33 & \num{1.61e+00} & \num{2.93e+05} & \num{3.92e+01} & \num{2.20e+00}\\ 
 & 2 & 46.71 & \num{2.06e+00} & \num{2.93e+05} & \num{4.58e+02} & \num{1.58e+00}\\ 
\hline
\multirow{2}{*}{61.75} & 1 & 49.00 & \num{1.80e+00} & \num{2.92e+05} & \num{4.41e+01} & \num{2.23e+00}\\ 
 & 2 & 47.20 & \num{1.26e+00} & \num{2.92e+05} & \num{2.47e+02} & \num{1.69e+00}\\ 
\hline
\multirow{2}{*}{62.75} & 1 & 49.67 & \num{2.14e+00} & \num{2.91e+05} & \num{4.92e+01} & \num{2.29e+00}\\ 
 & 2 & 47.53 & \num{1.91e+00} & \num{2.91e+05} & \num{3.05e+02} & \num{1.79e+00}\\ 
\hline
\multirow{2}{*}{63.75} & 1 & 50.34 & \num{2.66e+00} & \num{2.90e+05} & \num{8.39e+01} & \num{2.39e+00}\\ 
 & 2 & 47.67 & \num{1.56e+00} & \num{2.90e+05} & \num{1.47e+02} & \num{1.51e+00}\\ 
\hline
\multirow{2}{*}{64.25} & 1 & 50.67 & \num{2.72e+00} & \num{2.90e+05} & \num{7.76e+01} & \num{2.39e+00}\\ 
 & 2 & 47.94 & \num{1.46e+00} & \num{2.90e+05} & \num{1.85e+02} & \num{1.50e+00}\\ 
\hline
\multirow{2}{*}{64.75} & 1 & 51.01 & \num{2.99e+00} & \num{2.89e+05} & \num{9.99e+01} & \num{2.47e+00}\\ 
 & 2 & 48.00 & \num{1.25e+00} & \num{2.90e+05} & \num{1.60e+02} & \num{1.34e+00}\\ 
\hline
\multirow{3}{*}{65.75} & 1 & 51.66 & \num{3.44e+00} & \num{2.89e+05} & \num{1.87e+02} & \num{2.58e+00}\\ 
 & 2 & 48.16 & \num{1.16e-02} & \num{2.90e+05} & \num{4.28e+01} & \num{7.19e-01}\\ 
 & 3 & 44.89 & \num{1.11e+00} & \num{2.90e+05} & \num{3.24e+01} & \num{1.98e+00}\\ 
\hline
\multirow{2}{*}{66.25} & 1 & 52.00 & \num{3.64e+00} & \num{2.88e+05} & \num{3.32e+02} & \num{2.67e+00}\\ 
 & 2 & 48.27 & \num{1.16e+00} & \num{2.89e+05} & \num{2.57e+02} & \num{1.17e+00}\\ 
\hline
\multirow{2}{*}{66.75} & 1 & 52.32 & \num{3.75e+00} & \num{2.88e+05} & \num{1.65e+02} & \num{2.81e+00}\\ 
 & 2 & 48.47 & \num{2.55e+00} & \num{2.89e+05} & \num{2.67e+02} & \num{1.11e+00}\\ 
\hline
\multirow{3}{*}{67.25} & 1 & 52.65 & \num{3.80e+00} & \num{2.88e+05} & \num{1.13e+02} & \num{2.96e+00}\\ 
 & 2 & 48.71 & \num{4.70e-03} & \num{2.89e+05} & \num{3.33e+01} & \num{5.60e-01}\\ 
 & 3 & 44.40 & \num{1.22e+00} & \num{2.89e+05} & \num{7.32e+01} & \num{1.92e+00}\\ 
\hline
\multirow{2}{*}{67.75} & 1 & 52.99 & \num{3.91e+00} & \num{2.87e+05} & \num{1.28e+02} & \num{2.89e+00}\\ 
 & 2 & 45.20 & \num{1.57e+00} & \num{2.89e+05} & \num{2.19e+02} & \num{2.11e+00}\\ 
\hline
\multirow{3}{*}{68.25} & 1 & 53.31 & \num{3.97e+00} & \num{2.87e+05} & \num{2.54e+02} & \num{3.25e+00}\\ 
 & 2 & 49.15 & \num{8.31e-04} & \num{2.89e+05} & \num{5.60e+00} & \num{4.74e-01}\\ 
 & 3 & 44.24 & \num{1.35e+00} & \num{2.89e+05} & \num{4.31e+01} & \num{1.78e+00}\\ 
\hline
\multirow{2}{*}{68.75} & 1 & 53.63 & \num{3.94e+00} & \num{2.87e+05} & \num{2.21e+02} & \num{3.33e+00}\\ 
 & 2 & 44.54 & \num{1.52e+00} & \num{2.89e+05} & \num{8.84e+01} & \num{1.86e+00}\\ 
\hline
\multirow{2}{*}{69.25} & 1 & 53.97 & \num{4.08e+00} & \num{2.86e+05} & \num{2.26e+02} & \num{3.69e+00}\\ 
 & 2 & 44.08 & \num{1.64e+00} & \num{2.89e+05} & \num{9.49e+01} & \num{1.92e+00}\\ 
\hline
\multirow{3}{*}{69.75} & 1 & 54.29 & \num{4.20e+00} & \num{2.86e+05} & \num{3.90e+02} & \num{3.86e+00}\\ 
 & 2 & 44.31 & \num{4.69e-01} & \num{2.89e+05} & \num{2.71e+02} & \num{2.34e+00}\\ 
 & 3 & 44.31 & \num{1.84e+00} & \num{2.89e+05} & \num{4.88e+02} & \num{2.15e+00}\\ 
\hline
\multirow{2}{*}{70.25} & 1 & 54.62 & \num{4.72e+00} & \num{2.85e+05} & \num{1.76e+02} & \num{3.90e+00}\\ 
 & 2 & 43.59 & \num{1.62e+00} & \num{2.89e+05} & \num{9.45e+01} & \num{1.87e+00}\\ 
\hline
\multirow{3}{*}{70.75} & 1 & 54.94 & \num{4.89e+00} & \num{2.85e+05} & \num{2.18e+02} & \num{3.89e+00}\\ 
 & 2 & 49.77 & \num{2.19e-03} & \num{2.89e+05} & \num{4.92e+01} & \num{5.06e-01}\\ 
 & 3 & 43.49 & \num{8.05e-01} & \num{2.89e+05} & \num{8.72e+01} & \num{2.11e+00}\\ 
\hline
\multirow{3}{*}{71.00} & 1 & 55.11 & \num{5.02e+00} & \num{2.85e+05} & \num{1.96e+02} & \num{3.89e+00}\\ 
 & 2 & 49.80 & \num{4.43e-03} & \num{2.88e+05} & \num{8.28e+01} & \num{5.85e-01}\\ 
 & 3 & 43.41 & \num{8.16e-01} & \num{2.88e+05} & \num{7.41e+01} & \num{2.13e+00}\\ 
\hline
\multirow{3}{*}{71.25} & 1 & 55.26 & \num{5.73e+00} & \num{2.85e+05} & \num{1.25e+02} & \num{3.86e+00}\\ 
 & 2 & 49.22 & \num{5.90e-03} & \num{2.89e+05} & \num{1.30e+02} & \num{6.31e-01}\\ 
 & 3 & 42.61 & \num{7.94e-01} & \num{2.89e+05} & \num{6.93e+01} & \num{2.15e+00}\\ 
\hline
\multirow{3}{*}{71.50} & 1 & 55.42 & \num{5.39e+00} & \num{2.85e+05} & \num{7.80e+01} & \num{3.88e+00}\\ 
 & 2 & 49.73 & \num{8.12e-03} & \num{2.88e+05} & \num{1.34e+02} & \num{6.84e-01}\\ 
 & 3 & 43.06 & \num{7.21e-01} & \num{2.88e+05} & \num{3.11e+01} & \num{2.02e+00}\\ 
\hline
\multirow{3}{*}{71.75} & 1 & 55.59 & \num{5.97e+00} & \num{2.84e+05} & \num{2.94e+02} & \num{3.84e+00}\\ 
 & 2 & 49.31 & \num{8.68e-03} & \num{2.88e+05} & \num{1.61e+02} & \num{7.18e-01}\\ 
 & 3 & 42.48 & \num{4.83e-01} & \num{2.88e+05} & \num{7.81e+00} & \num{1.77e+00}\\ 
\hline
\multirow{3}{*}{72.00} & 1 & 55.74 & \num{5.85e+00} & \num{2.84e+05} & \num{2.36e+02} & \num{3.85e+00}\\ 
 & 2 & 49.58 & \num{1.27e-02} & \num{2.88e+05} & \num{1.73e+02} & \num{7.74e-01}\\ 
 & 3 & 42.63 & \num{7.34e-01} & \num{2.88e+05} & \num{4.65e+01} & \num{2.25e+00}\\ 
\hline
\multirow{3}{*}{72.25} & 1 & 55.91 & \num{7.37e+00} & \num{2.84e+05} & \num{6.03e+02} & \num{3.63e+00}\\ 
 & 2 & 48.19 & \num{1.38e-02} & \num{2.89e+05} & \num{1.94e+02} & \num{8.11e-01}\\ 
 & 3 & 41.57 & \num{4.18e-01} & \num{2.89e+05} & \num{6.72e+00} & \num{1.83e+00}\\ 
\hline
\multirow{3}{*}{72.50} & 1 & 56.07 & \num{7.32e+00} & \num{2.84e+05} & \num{6.56e+02} & \num{3.63e+00}\\ 
 & 2 & 48.41 & \num{1.30e+00} & \num{2.88e+05} & \num{2.43e+02} & \num{7.15e-01}\\ 
 & 3 & 41.66 & \num{5.45e-01} & \num{2.88e+05} & \num{1.00e+01} & \num{1.94e+00}\\ 
\hline
\multirow{3}{*}{72.75} & 1 & 56.24 & \num{7.77e+00} & \num{2.84e+05} & \num{8.91e+02} & \num{3.59e+00}\\ 
 & 2 & 48.11 & \num{1.35e+00} & \num{2.88e+05} & \num{2.73e+02} & \num{7.33e-01}\\ 
 & 3 & 41.39 & \num{5.85e-01} & \num{2.88e+05} & \num{1.48e+01} & \num{2.05e+00}\\ 
\hline
\multirow{3}{*}{73.00} & 1 & 56.39 & \num{8.29e+00} & \num{2.84e+05} & \num{1.44e+03} & \num{3.55e+00}\\ 
 & 2 & 42.48 & \num{3.83e-01} & \num{2.88e+05} & \num{2.81e+02} & \num{2.55e+00}\\ 
 & 3 & 42.48 & \num{1.74e+00} & \num{2.88e+05} & \num{1.03e+03} & \num{2.26e+00}\\ 
\hline
\multirow{3}{*}{73.25} & 1 & 56.55 & \num{8.91e+00} & \num{2.84e+05} & \num{1.75e+03} & \num{3.48e+00}\\ 
 & 2 & 42.16 & \num{4.45e-01} & \num{2.88e+05} & \num{3.16e+02} & \num{2.52e+00}\\ 
 & 3 & 42.16 & \num{1.75e+00} & \num{2.88e+05} & \num{9.38e+02} & \num{2.27e+00}\\ 
\hline
\multirow{3}{*}{73.50} & 1 & 56.72 & \num{9.98e+00} & \num{2.83e+05} & \num{2.12e+03} & \num{3.43e+00}\\ 
 & 2 & 46.34 & \num{1.31e+00} & \num{2.88e+05} & \num{2.65e+02} & \num{7.51e-01}\\ 
 & 3 & 40.11 & \num{4.73e-01} & \num{2.88e+05} & \num{1.52e+01} & \num{2.02e+00}\\ 
\hline
\multirow{3}{*}{73.75} & 1 & 56.87 & \num{1.04e+01} & \num{2.83e+05} & \num{3.24e+03} & \num{3.43e+00}\\ 
 & 2 & 46.09 & \num{1.30e+00} & \num{2.88e+05} & \num{2.66e+02} & \num{7.52e-01}\\ 
 & 3 & 39.92 & \num{4.49e-01} & \num{2.88e+05} & \num{1.37e+01} & \num{2.01e+00}\\ 
\hline
\multirow{3}{*}{74.75} & 1 & 57.51 & \num{1.27e+01} & \num{2.83e+05} & \num{3.83e+03} & \num{3.37e+00}\\ 
 & 2 & 44.46 & \num{1.18e-02} & \num{2.88e+05} & \num{2.15e+02} & \num{8.29e-01}\\ 
 & 3 & 38.68 & \num{4.35e-01} & \num{2.88e+05} & \num{2.08e+01} & \num{2.08e+00}\\ 
\hline
\multirow{3}{*}{75.00} & 1 & 57.68 & \num{1.35e+01} & \num{2.82e+05} & \num{1.69e+03} & \num{3.34e+00}\\ 
 & 2 & 44.20 & \num{5.50e+00} & \num{2.82e+05} & \num{4.97e+07} & \num{8.01e-01}\\ 
 & 3 & 38.34 & \num{1.27e+00} & \num{2.88e+05} & \num{1.87e+02} & \num{2.33e+00}\\ 
\hline
\multirow{3}{*}{75.25} & 1 & 57.84 & \num{1.33e+01} & \num{2.82e+05} & \num{1.85e+03} & \num{3.35e+00}\\ 
 & 2 & 44.51 & \num{5.66e+00} & \num{2.82e+05} & \num{4.95e+07} & \num{8.60e-01}\\ 
 & 3 & 38.49 & \num{1.67e+00} & \num{2.88e+05} & \num{1.60e+02} & \num{2.43e+00}\\ 
\hline
\multirow{3}{*}{75.50} & 1 & 57.99 & \num{1.39e+01} & \num{2.82e+05} & \num{1.40e+03} & \num{3.31e+00}\\ 
 & 2 & 44.10 & \num{5.49e+00} & \num{2.82e+05} & \num{5.02e+07} & \num{8.51e-01}\\ 
 & 3 & 38.25 & \num{1.30e+00} & \num{2.88e+05} & \num{1.92e+02} & \num{2.35e+00}\\ 
\hline
\multirow{2}{*}{76.25} & 1 & 58.47 & \num{1.59e+01} & \num{2.82e+05} & \num{1.87e+03} & \num{3.28e+00}\\ 
 & 2 & 42.18 & \num{1.72e+00} & \num{2.88e+05} & \num{3.58e+02} & \num{1.03e+00}\\ 
\hline
\multirow{2}{*}{76.50} & 1 & 58.63 & \num{1.70e+01} & \num{2.82e+05} & \num{5.42e+02} & \num{3.23e+00}\\ 
 & 2 & 41.28 & \num{1.69e+00} & \num{2.88e+05} & \num{2.89e+02} & \num{9.85e-01}\\ 
\hline
\multirow{2}{*}{76.75} & 1 & 58.79 & \num{1.81e+01} & \num{2.81e+05} & \num{8.88e+02} & \num{3.19e+00}\\ 
 & 2 & 40.39 & \num{1.61e+00} & \num{2.88e+05} & \num{2.01e+02} & \num{9.25e-01}\\ 
\hline
\multirow{2}{*}{77.00} & 1 & 58.96 & \num{1.90e+01} & \num{2.81e+05} & \num{1.11e+03} & \num{3.15e+00}\\ 
 & 2 & 39.57 & \num{2.26e+00} & \num{2.88e+05} & \num{1.44e+02} & \num{1.02e+00}\\ 
\hline
\multirow{2}{*}{77.25} & 1 & 59.10 & \num{2.03e+01} & \num{2.81e+05} & \num{9.58e+02} & \num{3.09e+00}\\ 
 & 2 & 38.43 & \num{1.99e+00} & \num{2.88e+05} & \num{8.77e+01} & \num{1.14e+00}\\ 
\hline
\multirow{2}{*}{77.50} & 1 & 59.27 & \num{2.13e+01} & \num{2.81e+05} & \num{9.91e+02} & \num{3.05e+00}\\ 
 & 2 & 37.61 & \num{1.75e+00} & \num{2.88e+05} & \num{7.18e+01} & \num{1.03e+00}\\ 
\hline
\multirow{2}{*}{77.75} & 1 & 59.43 & \num{2.25e+01} & \num{2.81e+05} & \num{1.23e+03} & \num{3.01e+00}\\ 
 & 2 & 36.66 & \num{1.55e+00} & \num{2.88e+05} & \num{4.95e+01} & \num{9.93e-01}\\ 
\hline
\multirow{2}{*}{80.00} & 1 & 60.84 & \num{4.16e+01} & \num{2.80e+05} & \num{2.07e+04} & \num{2.35e+00}\\ 
 & 2 & 19.03 & \num{8.13e-03} & \num{2.90e+05} & \num{3.41e-01} & \num{2.55e+00}\\ 
\hline

